Towards Engineering Fair and Equitable Software Systems for Managing Low-Altitude Airspace Authorizations

Small Unmanned Aircraft Systems (sUAS) have gained widespread adoption across a diverse range of applications. This has introduced operational complexities within shared airspaces and an increase in reported incidents, raising safety concerns. In response, the U.S. Federal Aviation Administration (FAA) is developing a UAS Traffic Management (UTM) system to control access to airspace based on an sUAS's predicted ability to safely complete its mission. However, a fully automated system capable of swiftly approving or denying flight requests can be prone to bias and must consider safety, transparency, and fairness to diverse stakeholders. In this paper, we present an initial study that explores stakeholders' perspectives on factors that should be considered in an automated system. Results indicate flight characteristics and environmental conditions were perceived as most important but pilot and drone capabilities should also be considered. Further, several respondents indicated an aversion to any AI-supported automation, highlighting the need for full transparency in automated decision-making. Results provide a societal perspective on the challenges of automating UTM flight authorization decisions and help frame the ongoing design of a solution acceptable to the broader sUAS community.

==> parkinglot.tex <==
% This is just Jane's scratch pad :-)

Challenging questions must be asked and answered to define the conditions under which it is safe for an sUAS to conduct its mission, what kind of data can be collected about sUAS and their operators, and what constitutes a fair decision. In current practice, operators seeking permission from the FAA to fly BVLOS or other cutting-edge missions, submit lengthy and detailed reports which take weeks or months of review, with an emphasis upon safety. However, developing, validating, and deploying an automated system to approve or reject such sUAS flight requests, is a complex, multi-faceted process which ultimately must
balance competing concerns including, but not limited to, safety, privacy, transparency, and fairness to diverse stakeholders. In this paper, we therefore report  on an initial exploratory study, the first of its kind, to understand user perspectives of a fairness automated UTM system and techniques for enhancing transparency. Results from our survey indicate that flight characteristics and environmental
conditions, such as those currently assessed in manual reviews, were perceived as most important, but that pilot and drone capabilities should also be considered.
Further, several survey respondents indicated aversion to any AI-supported automation at all, highlighting the need for full transparency in any automated decision making. Results from this survey provide a societal perspective on the challenges of automating UTM decisions, and frame ongoing design decisions witht he aim of developing a solution acceptable to the broader sUAS community and increasing the likelihood of its ultimate acceptance.
